RealToxicityPrompts: Evaluating Neural Toxic Degeneration in Language Models

Pretrained neural language models (LMs) are prone to generating racist, sexist, or otherwise toxic language which hinders their safe deployment. We investigate the extent to which pretrained LMs can be prompted to generate toxic language, and the effectiveness of controllable text generation algorithms at preventing such toxic degeneration. We create and release RealToxicityPrompts, a dataset of 100K naturally occurring, sentence-level prompts derived from a large corpus of English web text, paired with toxicity scores from a widely-used toxicity classifier. Using RealToxicityPrompts, we find that pretrained LMs can degenerate into toxic text even from seemingly innocuous prompts. We empirically assess several controllable generation methods, and find that while data- or compute-intensive methods (e.g., adaptive pretraining on non-toxic data) are more effective at steering away from toxicity than simpler solutions (e.g., banning "bad" words), no current method is failsafe against neural toxic degeneration. To pinpoint the potential cause of such persistent toxic degeneration, we analyze two web text corpora used to pretrain several LMs (including GPT-2; Radford et. al, 2019), and find a significant amount of offensive, factually unreliable, and otherwise toxic content. Our work provides a test bed for evaluating toxic generations by LMs and stresses the need for better data selection processes for pretraining.

==> sections/10-controllable-details.tex <==
% details on our AffectLM implementation
% training, spans, how do we get token-level scores




==> sections/17-old-discussion-ethics.tex <==
\label{sec:ethics}

% \maarteninline{copy pasted this from 5.4 (temporarily)}
% Furthermore, while \dapt and \pplm outperform all other techniques we evaluate, they are by far the most computationally expensive. \dapt involves updating all the parameters of the language model, which becomes less feasible with as the size of the model grows. \pplm involves backpropagation steps during inference, which \suchin{Noah: quantify?} heavily slows inference time. This suggests that there is more work to be done to build cheaper, faster detoxification techniques for pretrained language models that are as effective as the most expensive options.

\maarteninline{Can we make this broadly about our full results, including recs about steering methods etc.}


These issues seem to propagate into the downstream behavior of NLP models; all language models we evaluate that are trained on \webtext corpora have a high propensity to produce toxic generations (\S\ref{sec:toxicity_in_gen_models}). Furthermore, current detoxification techniques are unable to completely prevent toxic output (\S\ref{sec:controllable_solutions}). These results imply an urgent need for not only stronger model detoxification techniques, but also more effective methods to handle toxicity in pretraining data.

While the problem of building better detoxification solutions is difficult in its own right, the issue of how to best handle toxicity in pretraining corpora presents its own set of open ethical questions.

First, who has the power or responsibility to moderate the content that is included in the pretraining corpus? As language models become more prevalent in society, we echo \citet{Blodgett2020LanguageI} in calling for a re-imagination of the relationships between NLP researchers and community stakeholders of pretrained language models through value-sensitive \citep{Friedman2013ValueSD} or participatory \citep{DiSalvo2012CommunitiesPD} design. We advocate that researchers engage with affected populations to understand which sorts of data we should be including and why.

Furthermore, as with other bias measurements in NLP \citep{Jacobs2019MeasurementAF}, our measurements of toxicity are limited by the inherent biases of \perspective, as we detail in \S\ref{ssec:biases-toxicity-detection}.  Does the integration of automated toxicity classifiers entail possible censorship of voices that are more likely to be incorrectly flagged as toxic? Value-sensitive and/or participatory design principles could also be integrated into the evaluation framework to combat these issues. For example, future work may attempt to integrate humans-in-the-loop to improve the precision of our measurements of toxicity at-scale, or customize how toxicity is detected for specific groups of people. Though we focus on toxicity as our primary conceptualization of representational bias in this paper, the evaluation framework we propose can be used with other bias measurements, e.g., those of gender stereotyping \citep{Fast2016ShirtlessAD}, demographic misrepresentation \citep{Hovy2016TheSI}, or implied social biases \citep{sap2020socialbiasframes}.

The way that datasets are collected has a fundamental impact on the representational biases of NLP models \suchininline{CITE!!}. In \S\ref{sec:owtc-analyses}, we show that that examining \emph{sources} of toxic content can illuminate effective heuristics to reduce toxicity in the pretraining data, thus hopefully reduce the likelihood of toxic degeneration. However, this sort of research is only possible when source content is made available to researchers. Echoing works that emphasize transparency in NLP research \citep{Bender2018DataSF, Mitchell2019ModelCF}, we also urge researchers to make available \emph{all} information (e.g. original text, source URLs, timestamps, platform-specific metadata) surrounding pretraining data readily available for toxicity research. By making all data available, we have a better chance to understand how and why models engage in toxic degeneration, and in effect, how to better combat that behavior.


% incorporate insights from data statements (Bender & Friedman)

% who decides what is toxic & what to include (rope in some of the "let affected populations decide for themselves & allow for customization" Hannah wallach stuff?)
% reiterating issues with toxicity classifiers and potential censorship impact
% REC: think of other social biases that are present in data cite fast2016shirtless, sheng2019, sap2020socialbiasframes 

% \suchininline{Possible things to talk about here: 
% \begin{enumerate}
% \item Who gets to (and has the responsibility to) mediate content in pretraining data?
% \item Biases in toxicity classification may result in removing minority voices, since they are more likely to be flagged as toxic if mentioned
% \item ...
% \end{enumerate}
%  }




==> tables/precision_recall_naughty_words.tex <==
% INSULT SCORE: precision: 0.20182291666666666, recall: 0.5535714285714286, f1: 0.2958015267175573
% SEVERE TOXICITY SCORE: precision: 0.11675347222222222, recall: 0.766928011404134, f1: 0.2026556172897636
% TOXICITY SCORE: precision: 0.1591796875, recall: 0.6626016260162602, f1: 0.2566929133858268
% PROFANITY SCORE: precision: 0.19173177083333334, recall: 0.690504103165299, f1: 0.30012738853503185
% SEXUALLY EXPLICIT SCORE: precision: 0.2684461805555556, recall: 0.7844007609384908, f1: 0.39999999999999997
% FLIRTATION SCORE: precision: 0.2965494791666667, recall: 0.34230961923847697, f1: 0.31779069767441864
% IDENTITY ATTACK SCORE: precision: 0.1929253472222222, recall: 0.3185808994803799, f1: 0.24031898357775222
% THREAT SCORE: precision: 0.1557074652777778, recall: 0.26200474712433813, f1: 0.19533111005240592
% AVERAGE TOXICITY SCORE: precision: 0.15201822916666666, recall: 0.7428419936373277, f1: 0.25238695730499006


\begin{table}[t]
    \centering
    \begin{tabular}{cccc}
    \toprule
    \bf\textsc{Persp.}  Label  &\bf Recall$_{\text{NW}}$ & \bf Recall$_{\text{NW++}}$
    \\\midrule
    \textsc{Sexual} & 0.90 & 0.91 \\
    \toxicity & 0.89 & 0.90  \\
    \profanity & 0.88 & 0.89 \\
    \insult & 0.80 & 0.83 \\
    \flirtation & 0.72 & 0.73 \\
    \textsc{Iden. Attack} & 0.62 &  0.71 \\
    \threat & 0.52 & 0.59 \\
    \midrule
    \textsc{Avg.\textsubscript{std}} & 78.4$_{15.2}$ & 0.82$_{12.6}$ \\
    \bottomrule
    \end{tabular}
    \caption{Naughty word filtering (left column) has higher recall for toxicity categories like \sexexplicit, \profanity, and \toxicity, but very low recall for labels such as \identityattack and \threat. By additionally filtering documents from quarantined/banned subreddits, ideologically extreme news sources, and factually unreliable news sources (right column), we improve recall across all \perspective labels, especially \identityattack and \threat.}
    \label{tab:precision_recall}
\end{table}



==> tables/toxicity_bias_correlation.tex <==
% INSULT SCORE: precision: 0.20182291666666666, recall: 0.5535714285714286, f1: 0.2958015267175573
% SEVERE TOXICITY SCORE: precision: 0.11675347222222222, recall: 0.766928011404134, f1: 0.2026556172897636
% TOXICITY SCORE: precision: 0.1591796875, recall: 0.6626016260162602, f1: 0.2566929133858268
% PROFANITY SCORE: precision: 0.19173177083333334, recall: 0.690504103165299, f1: 0.30012738853503185
% SEXUALLY EXPLICIT SCORE: precision: 0.2684461805555556, recall: 0.7844007609384908, f1: 0.39999999999999997
% FLIRTATION SCORE: precision: 0.2965494791666667, recall: 0.34230961923847697, f1: 0.31779069767441864
% IDENTITY ATTACK SCORE: precision: 0.1929253472222222, recall: 0.3185808994803799, f1: 0.24031898357775222
% THREAT SCORE: precision: 0.1557074652777778, recall: 0.26200474712433813, f1: 0.19533111005240592
% AVERAGE TOXICITY SCORE: precision: 0.15201822916666666, recall: 

\begin{table}[t]
    \centering
    \begin{tabular}{cc}
    \toprule
    \bf\textsc{Persp.}  Label & \bf Factual Reliability  \\\midrule
    \textsc{Sexual} & -0.11 \\
    \toxicity & -0.20 \\
    \profanity & -0.19 \\
    \insult & -0.21 \\
    \flirtation & -0.08 \\
    \textsc{Iden. Attack} & -0.19 \\
    \threat & -0.15 \\
    \midrule
    \textsc{Avg.\textsubscript{std}} & -0.16$_{0.04}$ \\
    \bottomrule
    \end{tabular}
    \caption{Spearman correlation between \toxicity and Factual reliability in news articles of \openwebtext.}
    \label{tab:factual_reliability_toxicity}
\end{table}



==> tables/toxicity_breakdown.tex <==
% Insult Score 0.0336
% Severe Toxicity Score 0.01403
% Toxicity Score 0.02214
% Profanity Score 0.02559
% Sexually Explicit Score 0.03154
% Flirtation Score 0.07984
% Identity Attack Score 0.05581
% Threat Score 0.05477
% Average Toxicity Score 0.01888
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{cc}
    \toprule
    \bf\textsc{Persp.}  Label & \bf Percentage of \openwebtext  \\\midrule
    \textsc{Sexual} & 3.2\% \\
    \toxicity & 2.2\%\\
    \profanity & 2.6\% \\
    \insult & 3.4\% \\
    \flirtation & 8.0\%\\
    \textsc{Sev. Toxicity} & 1.4\% \\
    \textsc{Iden. Attack} & 5.6\% \\
    \threat & 5.5\% \\
    \bottomrule
    \end{tabular}
    \caption{Breakdown of toxicity in \openwebtext by category.}
    \label{tab:precision_recall}
\end{table}


